Learning Robotic Assembly from CAD

In this work, motivated by recent manufacturing trends, we investigate autonomous robotic assembly. Industrial assembly tasks require contact-rich manipulation skills, which are challenging to acquire using classical control and motion planning approaches. Consequently, robot controllers for assembly domains are presently engineered to solve a particular task, and cannot easily handle variations in the product or environment. Reinforcement learning (RL) is a promising approach for autonomously acquiring robot skills that involve contact-rich dynamics. However, RL relies on random exploration for learning a control policy, which requires many robot executions, and often gets trapped in locally suboptimal solutions. Instead, we posit that prior knowledge, when available, can improve RL performance. We exploit the fact that in modern assembly domains, geometric information about the task is readily available via the CAD design files. We propose to leverage this prior knowledge by guiding RL along a geometric motion plan, calculated using the CAD data. We show that our approach effectively improves over traditional control approaches for tracking the motion plan, and can solve assembly tasks that require high precision, even without accurate state estimation. In addition, we propose a neural network architecture that can learn to track the motion plan, and generalize the assembly controller to changes in the object positions.

==> old_text.tex <==
% Robot controllers that can quickly adapt to changes in a product design, or that can learn to perform the assembly automatically from a CAD specification, have the potential to revolutionize robotic assembly, and are required for future developments such as industry 4.0 \cite{lasi2014industry}.

% There are challenges: assembly task often are contact-rich, and require handling friction and contact as part of the solution. For example, think of mounting a hard drive into a desktop chassis, or assembling a gear onto a shaft. 
% Unfortunately, accurate modelling of dynamics that involve friction and contacts is difficult, making classical control techniques not suitable. (???)

% Current approaches for automatically designing controllers rely on either: motion planning using the geometrical CAD models + trajectory following control, or model based/model free RL. Motion planning methods do not account for dynamics, making them suboptimal for contact rich domains. RL doesn't use the geometry information, and is sample inefficient, and does not generalize well to new domains.

% In this work we combine CAD-based motion planning with RL to get the best of both worlds.


% We show that our approach can generalize better than SOTA RL methods, and learn quickly on the PR2 robot. In tasks that are contact-rich, our approach performs better than standard motion planning + tracking.



% combination of planning and learning: typically trajectories are acquired from human demonstration 
% \cite{pastor2009learning}
% \cite{mulling2013learning}


% Kinematic motion planning \cite{lavalle2006planning,latombe2012robot} uses a geometric model of the task to compute a motion plan that avoids obstacles. In order to execute the motion plan, a tracking controller such as a PD 
% related work:
% 1. Kinematic motion planning - can work well if contacts can be avoided, and using a high accuracy controller. This is difficult in many real-world applications. In particular, the iterative learning that we use enables fitting the controller to the real-world scenario (reword this sentence).
% 2. Iterative learning control (ILC) - we are actually doing ILC in the ILQR stage, however, the NN learn to generalize to different trajectories.
% 3. GPS - gets stuck in local minima since the complete trajectory is not given. Can use waypoints, but those need to be carefully defined manually. We automatically generate the trajectory from the CAD data.

% Our experiments should show improvement over (1-3). For (2), we just need to show zero-shot generalization to new trajectories.

% one shot imitation learning

% \cite{pastor2009learning} - imitation learning of skill using DMPs - requires human demonstration. Our method doesn't require human feedback (except for setting the target, which can be relaxed with better sensing/vision).

% dynamic motion planning - needs contact / friction dynamics, which is hard.


